Investigating Interaction Modes and User Agency in Human-LLM Collaboration for Domain-Specific Data Analysis

Despite demonstrating robust capabilities in performing tasks related to general-domain data-operation tasks, Large Language Models (LLMs) may exhibit shortcomings when applied to domain-specific tasks. We consider the design of domain-specific AI-powered data analysis tools from two dimensions: interaction and user agency. We implemented two design probes that fall on the two ends of the two dimensions: an open-ended high agency (OHA) prototype and a structured low agency (SLA) prototype. We conducted an interview study with nine data scientists to investigate (1) how users perceived the LLM outputs for data analysis assistance, and (2) how the two test design probes, OHA and SLA, affected user behavior, performance, and perceptions. Our study revealed insights regarding participants' interactions with LLMs, how they perceived the results, and their desire for explainability concerning LLM outputs, along with a noted need for collaboration with other users, and how they envisioned the utility of LLMs in their workflow.

==> README.tex <==

iui24.tex: initial submission. rejected.


files 02-05 were created after iui 24 submission.



==> backup.tex <==

\subsection{Quotes}

\begin{quote}
    \textit{
    I think this is too many rankings. Like three question, five options... Maybe something like just a thumbs up, thumbs down, would be easier. (P1)
    }
\end{quote}

\begin{quote}
    \textit{
    It completely over promised the delivery of the machine learning model for the construction lot. This of course makes me very unsatisfied because with a ChatGPT similar upfront, I already know that it's not capable of it and hence I don't ask it to do it. But since the LLM model, like after the enhancing of the prompted, suggested I should ask it to deliver me something, I would not been very unsatisfied, if it delivered at least something and the model had a bad performance. I mean, it would have surprised me very much if it would come up with a model, a generative model for the time series data that performs very well. But I'm very unsatisfied that it does not give me a model at all and also does not explain to me I did not give me a model. (P6)
    }
\end{quote}

\begin{quote}
    \textit{
    I think for the first time even for us to think what to tell to customer from this graph, it takes a little bit time to think how to explain. But here, if we read these insights, it gives some tips what can make sense... 
    according to us and how it can be maybe better articulated to customers, this insights, to start something, it is really good, but maybe a little bit more articulation or a little bit more information added, additional might be required when we are telling to the user. But I think this insights are helpful. (P8)
    }
\end{quote}



\subsection{Challenges of Domain Knowledge Data Science Job}

\subsubsection{Too Much Time Spent on Communication with Customers}

\begin{quote}
    \textit{
    Honestly the biggest factor probably is good communication between the clients and us. It's not like a technical thing, but that's where I found the biggest driver of success or failure in a project is how good the communication is with our users. (P2)
    }
\end{quote}


Requests that are trivial to implement; there are direct options they can use. Very little research involved. So they want to solve these things quickly. 
Large scale plots with millions of samples
Don’t have specific knowledge / bandwidth 


\subsubsection{Domain Knowledge is not Well-documented}

\subsubsection{Redundant Tasks}

Many participants mentioned that sometimes their job is quite repetitive.
P3 have worked closely with clients who have limited experience with data science but request machine learning models to help them make predictions.
The data provided by clients was often dirty or insufficient, and clients often have high expectations.
\textit{
"The predictions are not useful or things they already know, so you have to clean the data and iterate several times over that. It's very short term, but you have to make a lot of visualizations really fast."
}
P3 expresses the need for a tool to assist with common data science operations such as coding and cross-validation.

\begin{quote}
    \textit{
    I had to very quickly get a sample data and come up with why. So that was very closely working with plant people because as you get the data, they don't think that data is relevant, so you have to join the day, more data, and you make a model. The predictions are not useful or things they already know, so you have to clean the data and iterate several times over that. So it's very short term, but you have to make a lot of visualizations really fast. 
    }
\end{quote}

\begin{quote}
    \textit{
    they promise you, they swear that it is a good data. Most data is junk. It's a ton of missing variables, and there's a ton of things they already knew and it's not relevant. So they, you need to iterate mm-hmm. <affirmative>, so you need that person right next to you because it's trivial for them to help you do it, but you by yourself, you don't have the domain knowledge. You can't, you can't do it yourself. (P3)
    }
And what the tables we receive, they're full of measurements and names that don't mean anything to us. For a person that knows the product, these measurements are obvious. 
\end{quote}

\section{Study 2: Expert-in-the-loop V.S. Automatic Approach}
How do expert-in-the-loop differ from automatic exemplar generation?
In this study, we want to answer the following research question: 
\textbf{
Do exemplars make LLMs perform better in domain-specific data analysis?
}

\subsection{nvDomainBench}

We created a domain knowledge benchmark dataset from nvBench \cite{Luo2021-nvBench}. 
nvBench is a dataset for NL2VIS tasks, which covers 105 domains, supports seven common types of visualizations, and contains 25,750 (NL, VIS) pairs.
Each task contains...

\subsection{Experiment Design}

Condition 1: Human select + edit 1 variation, select 1 exemplar
Condition 2: LLM pick select 1 variation
Condition 3: same as 2, use detailed DK
Each task is done by >= 2 human participants and done by LLM >= 2 times. Pick the highest score for human/LLM. 

Meta Kaggle
\footnote{\url{https://www.kaggle.com/datasets/kaggle/meta-kaggle}}




\section{Discussion}
\subsection{Advanced LLM-powered Agent Capacities}

\subsubsection{Domain Knowledge Retrieval from Documentation}

\subsubsection{Multimodal Domain Knowledge Sharing}

\subsection{Transparency and Explainability}

\subsubsection{Explainability}

\subsubsection{How to Build Trust among Users?}

Most of the participants have experience with LLMs and they are aware of the risk of AI technologies. From our interview study, they still have positive attitudes towards the LLM-based applications. Many participants revealed that they have seen the values in the tools. 


\subsection{Use of LLM}

LLM (ChatGPT) is used in the paper in the following tasks.
(1) Two researchers created \datasetname{} with the assistance of ChatGPT to augment artificial domain knowledge, polish domain knowledge definitions, and generate code as exemplars. Details please see Section \ref{sec:quant_study}
(2) ChatGPT is employed to polish the grammar of this draft. No text is generated purely by LLM.

% \todo{Required by ACM}

\subsection{Collaborative System for Users with Various Expertise Level}

In the interview study, we talked to data scientists who are currently working on domain-specific data. Even though many of them have many years of experience in this domain, they still consider themselves as "domain novice", as they do not work in the environments where data is generated.
During the interview, many of them suggested that the tool will have a great value for domain experts who have rich knowledge about the domain but not much experience with data analysis.

We organized a quadrant of potential users based on their expertise in specific domain and data science, as Figure \ref{fig:user_quadrant} shows.
